Stopping Criteria for, and Strong Convergence of, Stochastic Gradient Descent on Bottou-Curtis-Nocedal Functions

Stopping criteria for Stochastic Gradient Descent (SGD) methods play important roles from enabling adaptive step size schemes to providing rigor for downstream analyses such as asymptotic inference. Unfortunately, current stopping criteria for SGD methods are often heuristics that rely on asymptotic normality results or convergence to stationary distributions, which may fail to exist for nonconvex functions and, thereby, limit the applicability of such stopping criteria. To address this issue, in this work, we rigorously develop two stopping criteria for SGD that can be applied to a broad class of nonconvex functions, which we term Bottou-Curtis-Nocedal functions. Moreover, as a prerequisite for developing these stopping criteria, we prove that the gradient function evaluated at SGD's iterates converges strongly to zero for Bottou-Curtis-Nocedal functions, which addresses an open question in the SGD literature. As a result of our work, our rigorously developed stopping criteria can be used to develop new adaptive step size schemes or bolster other downstream analyses for nonconvex functions.

==> section/stopping_criteria.tex <==
As discussed in \S\ref{section-rigorous}, recall the key challenges related to estimated stopping criteria:
establishing that the underlying deterministic stopping criterion will be triggered;
establishing that the estimated stopping criterion will be triggered;
establishing false positive control;\footnote{Recall that a false positive occurs when the estimated stopping criterion is triggered, but the underlying deterministic stopping criterion, if it could be evaluated, would not have been triggered.} and
establishing false negative control.\footnote{Recall that a false negative occurs when the estimated stopping criterion is not triggered, but the underlying deterministic stopping criterion, if it could be evaluated, would have been triggered.}

We have addressed the first challenge in Corollary \ref{corollary-convergence} when the underlying deterministic stopping criteria relies on the gradient functions becoming sufficiently small in norm. Therefore, we now address whether the estimated stopping criterion will be triggered, and the issue of false negative control. We again underscore that while the probability of false positives can be controlled using the techniques discussed below, such bounds would be rather coarse and would not be useful in the typical optimization context where a false positive would be particularly insidious. 






Just as we observed for the deterministic stopping criterion, we can study whether the estimated stopping criterion is triggered using several distinct notions (e.g., triggered with probability one, triggered in probability, triggered with high probability). In this work, we address the more stringent standard of whether the estimated stopping criterion is triggered with probability one, as we formalize now.

\begin{definition}
A stopping criterion is said to be triggered if the probability of satisfying the stopping criteria in finite time is equal to one. 
\end{definition}

For practical purposes, we also  

With this definition, we will describe three scenarios under which we will rigorously develop whether a stopping criterion is triggered and control over false negatives. Then, we will present five stopping criteria. For three of them, we will rigorously demonstrate that they are detectable and how they control false negatives. We summarize the results in Table \ref{table-summary} with an empty cell indicating that the property is not established for the given criteria under the given scenario.

\begin{table}[ht]
\caption{A summary of detectability and false negative control results for the five stopping criteria and the three scenarios. An empty cell indicates that neither detectability nor false negative control for the stopping criteria was established.}
\label{table-summary}       % Give a unique label
\centering
\begin{tabular}{@{}lccc@{}}
\toprule\noalign{\smallskip}
Criteria & Scenario (a) & Scenario (b) & Scenario (c) \\ \noalign{\smallskip}\midrule\noalign{\smallskip}
\ref{stop-dg} & Proposition \ref{prop-SC-1-detect} & Proposition \ref{prop-SC-1-detect} & Proposition \ref{prop-SC-1-detect} \\
\ref{stop-mean-est} & Proposition \ref{prop-SC-2-detect-fn} & Proposition \ref{prop-SC-2-detect-fn} & Proposition \ref{prop-SC-2-detect-fn} \\
\ref{stop-mean-dep} &            &  &  \\
\ref{stop-vote-ind} &  & Proposition \ref{prop-SC-4-detect-fn} & Proposition \ref{prop-SC-4-detect-fn} \\
\ref{stop-vote-dep} \\
\noalign{\smallskip}\bottomrule
\end{tabular}
\end{table}
\marginnote{Rev, Num 9}[-5cm]



\subsection{Stopping Criteria by Gradient Estimation}

The most natural extension from deterministic, gradient-based stopping criteria to the stochastic case is to apply deterministic stopping criteria to either a periodic evaluation of the deterministic gradient (when feasible, e.g., \cite{johnson2013}), or to an estimate of the deterministic gradient over an independent sample. These two stopping criteria are stated below.

\condition{stop-dg}{Let $\epsilon > 0$. Let $\lbrace T_j \rbrace$ be a sequence of positive-valued, strictly increasing, finite stopping times with respect to $\lbrace \mathcal{F}_k \rbrace$. Then, the SGD iterates are stopped at iterate $T_J$ where
$$J = \min \left\lbrace j \geq 1: \norm{ \dot{F}(\beta_{T_j})}_2 \leq \epsilon\right\rbrace.$$}{SC-0}



\begin{remark}
Letting $\lbrace T_j \rbrace$ be deterministic and $\lbrace N_j \rbrace$ be deterministic is allowed in both stopping criteria. By using stopping times, we allow for greater generality of these stopping criteria as they can be adaptive to the behavior of the sequence.
\end{remark}

In both criteria, we evaluate the stopping criteria at strictly increasing stopping times, which ensures that we are not repeating the evaluation of the stopping criteria at the same iterate (as this can be represented by simply increasing the value of $N_j$ and would be redundant). Moreover, our condition that $\lbrace T_j \rbrace$ is increasing supplies the following instrumental result that is a direct consequence of Corollary \ref{corollary-convergence}.



We see that Corollary \ref{corollary-ST-converge} implies that \ref{stop-dg} is detectable; that is, it will be triggered in finite time under the BCN conditions. Thus, it applies to all three scenarios. 

\begin{proposition} \label{prop-SC-1-detect}
Let $F$ be a Bottou-Curtis-Nocedal function (\S \ref{subsection-bcn-specification}) and let $\lbrace \beta_k \rbrace$ be the iterates generated by Stochastic Gradient Descent satisfying \ref{prop-sympd} to \ref{prop-mineig} (\S \ref{subsection-sgd}). If the SGD iterates are subject to \ref{stop-dg} for some $\epsilon > 0$, then \ref{stop-dg} is detectable (i.e., $\condPrb{ T_J < \infty}{\mathcal{F}_0} = 1$ with probability one.)
\end{proposition}
\begin{proof}
We will drop the $\mathcal{F}_0$ conditioning for simplification. 
\end{proof}

Given that we are directly evaluating $\Vert \dot{F}(\beta_{T_j}) \Vert_2$, \ref{stop-dg} has no issues concerning false negatives or positives. Unfortunately, the story is not the same for \ref{stop-mean-est}. To understand \ref{stop-mean-est}, we will first need the following lemma.


With this lemma, the following result states when \ref{stop-mean-est} is detectable and how the false negative probability is controlled.


A criticism of both \ref{stop-dg} and \ref{stop-mean-est} is that the effort required to evaluate them is nearly identical to updating the parameter by the SGD method in order to achieve, presumably, an iterate that is closer to a stationary point. To address this criticism, we consider the following stopping criteria which makes use of information that is already computed in order to update the iterates. However, we will not address the detectability nor control over the false negative probability as it requires developing a maximal inequality that will be addressed in future work.

\condition{stop-mean-dep}{Let $\epsilon > 0$. Let $\lbrace T_j \rbrace$ be a sequence of positive-valued, strictly increasing, finite stopping times with respect to $\lbrace \mathcal{F}_k \rbrace$. Let $\lbrace N_j \rbrace$ be $\mathbb{N}$-valued random variables such that $N_j$ is measurable with respect to $\mathcal{F}_{T_j}$. Let $\bar \gamma \in (0,1)$ and let $\lbrace \gamma_j \rbrace$ be $(0,\bar \gamma)$-valued random variables such that $\gamma_j$ is measurable with respect to $\mathcal{F}_{T_j}$. The SGD iterates are stopped at iterate in $T_J+N_J-1$, where
$$
J = \min\left\lbrace j \geq 1 : \frac{1}{N_j}\norm{ \sum_{i\in I_j} \dot{f}(\beta_i,X_{i+1})}_2 \leq \epsilon  \right\rbrace,
$$
where $I_j = \lbrace T_j,T_j+1,\ldots,T_{j}+N_j - 1 \rbrace$.}{SC-3}

\subsection{Stopping Criteria by Majority Vote}

In the preceding discussion, we considered stopping criteria based on estimating the deterministic gradient, which are natural extensions of deterministic stopping criteria. However, we collecting this information is in some sense too much: we are simply trying to make an up-down decision about whether convergence has occurred, why should we not simply design a stopping criteria that exploits this structure directly? The following stopping criteria take this exact approach. In effect, the following stopping criteria test each stochastic gradient against some condition and then use the majority decision (as determined by a threshold) to determine whether to stop or to continue the iterates. The first stopping criteria, \ref{stop-vote-ind}, leverages independent samples, and would face the same aforementioned criticisms as \ref{stop-mean-est}. The second stopping criteria, \ref{stop-vote-dep}, uses the samples that generate the iterate sequence and avoid these criticisms. 



\condition{stop-vote-dep}{Let $\epsilon > 0$. Let $\lbrace T_j \rbrace$ be a sequence of positive-valued, strictly increasing, finite stopping times with respect to $\lbrace \mathcal{F}_k \rbrace$. Let $\lbrace N_j \rbrace$ be $\mathbb{N}$-valued random variables such that $N_j$ is measurable with respect to $\mathcal{F}_{T_j}$. Let $\bar \gamma \in (0,1)$ and let $\lbrace \gamma_j \rbrace$ be $(0,\bar \gamma)$-valued random variables such that $\gamma_j$ is measurable with respect to $\mathcal{F}_{T_j}$. The SGD iterates are stopped at iterate $T_J+N_J-1$, where
$$
J = \min\left\lbrace j \geq 1 : \frac{1}{N_j} \sum_{i\in I_j} \1{ \norm{\dot f (\beta_{i}, X_{i+1})}_2 \leq \epsilon} \geq \gamma_j \right\rbrace,
$$
where $I_j = \lbrace T_j,T_j+1,\ldots,T_{j}+N_j - 1 \rbrace$.}{SC-5}

The following supplies an analogue of Lemma \ref{lemma-prob-bound} to the stopping criteria specified in \ref{stop-vote-ind}. The result about detectability and control over the false negative probability follows.



\begin{proposition} \label{prop-SC-4-detect-fn}
Let $F$ be a Bottou-Curtis-Nocedal function (\S \ref{subsection-bcn-specification}) and let $\lbrace \beta_k \rbrace$ be the iterates generated by Stochastic Gradient Descent satisfying \ref{prop-sympd} to \ref{prop-mineig} (\S \ref{subsection-sgd}).

\textbf{Scenario (b):} Suppose that $C_1 = 0$ in \ref{condition-noise-grad}. Let $\rho \in (0,1)$. If the SGD iterates are subject to \ref{stop-vote-ind} for some $\epsilon > 0$, then \ref{stop-vote-ind} is detectable. Moreover, when 
\begin{equation}
\norm{ \dot{F}(\beta_{T_j})}_2 \leq \epsilon \sqrt{ \frac{\rho(1-\bar{\gamma})}{C_2 + 1} },
\end{equation}
then the probability of a false negative is controlled by
$\exp( - 2N_j (1-\rho)^2(1-\bar{\gamma})^2)$.

\textbf{Scenario (c):} Suppose \ref{condition-tail-pareto} holds. Let $\rho \in (0,1)$. If the SGD iterates are subject to \ref{stop-mean-est} for some 
\begin{equation}
0 < \epsilon \leq \pi_1 \pi_3 [\rho (1 - \bar{\gamma})]^{1/\pi_2},
\end{equation}
then \ref{stop-vote-ind} is detectable. Moreover, when
\begin{equation}
\norm{ \dot{F}(\beta_{T_j})}_2 \leq \frac{\epsilon}{\pi_3} \left[ \rho (1 - \bar{\gamma})  \right]^{1/\pi_2}
\end{equation}
then the probability of a false negative is controlled by $\exp( - 2N_j (1-\rho)^2(1-\bar{\gamma})^2)$.
\end{proposition}
\begin{proof}
The proof proceeds just as in Proposition \ref{prop-SC-2-detect-fn}. Therefore, it is sufficient to prove the lower bound on the true positive probability for each scenario.

\textbf{Scenario (b):} For $j$ satisfying the hypotheses, Lemma \ref{lemma-prob-bound} implies
\begin{equation}
\condPrb{ \norm{ \dot{f}(\beta_{T_j},X) }_2 \leq \epsilon}{\mathcal{F}_{T_j}} \geq 1 - \rho( 1 - \bar{\gamma}) > 0.
\end{equation} 
Therefore,
\begin{align}
\Delta_j &:= \gamma_j - \condPrb{ \norm{ \dot{f}(\beta_{T_j},X) }_2 \leq \epsilon}{\mathcal{F}_{T_j}} \\
		 &\leq \bar{\gamma} - 1 + \rho(1 - \bar{\gamma}) \\
		 &= (1 - \rho)(\bar{\gamma} - 1) \\
		 &< 0.
\end{align}
Applying Lemma \ref{lemma-prob-conc},
\begin{equation}
\begin{aligned}
&\condPrb{ \frac{1}{N_j} \sum_{i=1}^{N_j} \1{ \norm{ \dot{f}(\beta_{T_j},Z_{ij})}_2 \leq \epsilon} \geq \gamma_j }{\mathcal{F}_{T_j}}  \\
&\quad\geq 1 - \exp\left(-2N_j (1 - \rho)^2(1 -\bar{\gamma})^2\right).
\end{aligned}
\end{equation}

\textbf{Scenario (c):} For $j$ satisfying the hypotheses, note that $\pi_3 \Vert \dot{F}(\beta_{T_j}) \Vert_2 \leq \epsilon_3$. Therefore, applying Lemma \ref{lemma-prob-bound} with \ref{condition-tail-pareto}, 
\begin{equation}
\condPrb{ \norm{ \dot{f}(\beta_{T_j},X) }_2 \leq \epsilon}{\mathcal{F}_{T_j}} \geq 1 - \rho( 1 - \bar{\gamma}) > 0.
\end{equation} 
The remainder of the proof is identical to Scenario (b). \qed
\end{proof}

Just as for \ref{stop-mean-dep}, we will not address the whether \ref{stop-vote-dep} is detectable nor how we control its false negative probability. Again, such a result requires establishing a maximal inequality, which we intend to address in future efforts. 


==> table/conditions.tex <==
\begin{longtable}{@{}p{1.5in}p{2.95in}@{}} \toprule 
\textbf{Name} & \textbf{Description}\\ \midrule 
Limited Iterate Space & Either by assuming a convex component on the objective function \cite{ghadimi2016,reddi2016b,li2018,lei2018}, level-boundedness of the objective function that products a closed, convex iterate space \cite{huang2017}, or directly assuming closedness, convexity or boundedness \cite{ma2017,wang2019}, the iterate sequence $\lbrace \theta_k \rbrace$ generated by the algorithm is limited to a nice (e.g., compact) subset of $\mathbb{R}^p$. \\ \midrule
Uniformly bounded of $f$ with probability one 
& There exists $C > 0$ such that $$\Prb{ \bigcap_{\theta} \left\lbrace | f(\theta, X) | \leq C \right\rbrace } = 1.$$
See \cite{zhou2018,hu2017}. \\ \midrule
Uniformly Lipschitz continuous of $f$ with probability one 
& There exists a $C > 0$ such that  $$\Prb{ \bigcap_{\theta,\psi} \left\lbrace \frac{| f(\theta,X) - f(\psi,X) |}{\norm{\theta-\psi}_2} \leq C \right\rbrace } = 1.$$ See \cite{zhou2018,park2019}.\\ \midrule 
Uniformly bounded $\dot{f}$ with probability one &
There exists a $C > 0$ such that $$\Prb{ \bigcap_{\theta} \left\lbrace \norm{ \dot{f}(\theta,X) }_2 \leq C \right\rbrace }  = 1.$$ 
See \cite{ma2017}. \\ \midrule
Lipschitz continuous $F$ & There exists a $C > 0$ such that $\forall \theta, \psi$, 
$$|F(\theta) - F(\psi)| \leq L \norm{ \theta - \psi}_2.$$
See \cite{ghadimi2016} \\ \midrule 
Uniformly bounded second moment of $\dot{f}$ &
There exists a $C > 0$ such that $\forall \theta$,
$$ \E{ \norm{\dot{f}(\theta,X)}_2^2 } \leq C.$$ \\ \midrule
Uniform Lipschitz continuity of $\dot{f}$ with probability one &
There exists a $C > 0$ such that
$$\Prb{ \bigcap_{\theta,\psi} \left\lbrace \frac{\norm{ \dot{f}(\theta,X) - \dot{f}(\psi,X) }_2}{\norm{\theta-\psi}_2} \leq C  \right\rbrace } = 1.$$ \\ \midrule
Uniform Lipschitz continuity of $\dot F$ &
There exists a $C > 0$ such that $\forall \theta, \psi$,
$$ \norm{ \dot F(\theta) - \dot F(\psi)}_2 \leq C \norm{ \theta - \psi}_2.$$ \\ \midrule
Uniformly bounded noise model with probability one &
There exists a $C > 0$ such that
$$ \Prb{ \bigcap_{\theta} \left\lbrace \norm{\dot f(\theta,X) - \dot F(\theta)}_2 \leq C \right\rbrace } = 1.$$ \\ \midrule
Uniformly bounded variance of noise model &
There exists a $C > 0$ such that $\forall \theta$,
$$ \norm{ \var{\dot f(\theta,X)} }_2 \leq C.$$
\end{longtable}
